DIALECTBENCH: A NLP Benchmark for Dialects, Varieties, and Closely-Related Languages

Language technologies should be judged on their usefulness in real-world use cases. An often overlooked aspect in natural language processing (NLP) research and evaluation is language variation in the form of non-standard dialects or language varieties (hereafter, varieties). Most NLP benchmarks are limited to standard language varieties. To fill this gap, we propose DIALECTBENCH, the first-ever large-scale benchmark for NLP on varieties, which aggregates an extensive set of task-varied variety datasets (10 text-level tasks covering 281 varieties). This allows for a comprehensive evaluation of NLP system performance on different language varieties. We provide substantial evidence of performance disparities between standard and non-standard language varieties, and we also identify language clusters with large performance divergence across tasks. We believe DIALECTBENCH provides a comprehensive view of the current state of NLP for language varieties and one step towards advancing it further. Code/data: https://github.com/ffaisal93/DialectBench

==> MT.tex <==


\onecolumn

\begin{center}




\begin{longtable}{lllrr}
\caption{MT with references}
\label{tab:MT}\\
\toprule
     Language group &      Language Pairs  &  NLLB-600M\_bleu & NLLB-1.3B\_bleu  \\
\midrule
\endfirsthead
\caption[]{} \\
\toprule
    %&&&\multicolumn{2}{c}{finetune}&\multicolumn{2}{c}{zeroshot}\\
 %  lang-group & tgt &      src &       bert & xlmr &  bert &  xlmr \\
\midrule
\endhead
\midrule

\midrule
\endfoot

\bottomrule
\endlastfoot
\multirow{25}{*}{Turkish} & ru-ba  &     43.61 &     43.61  \\

& ba-ru & 51.15 \\
& en-tr  \\
& tr-en  \\
& az-tr   & 21.77& 25.49\\
& kk-en  & 31.02\\
& az-en    & 29.08 & 32.50\\
& ru-uz  & 51.47\\
& en-kk  & 23.76\\
& en-uz  & 37.64 \\
& tr-az  & 22.93\\
& en-az  & 27.87\\
& uz-ru  & 54.71\\
& ru-ky  & 18.32\\
& ky-ru  & 22.64 & 26.60\\
& ky-en  & 27.24\\
& en-ky  & 18.85 \\
& uz-en  & 40.65\\
& kaa-en  & 32.48 & 40.39\\
& sah-en & 15.16 & 29.00 \\
& ba-en     & 30.78 & 36.76 \\
& en-kaa & 19.87\\
& sah-ru  & 30.27 & 23.65\\
& ru-sah & 7.53 & 14.86\\
& en-ba   & 25.00 & 38.21\\
& en-sah & 2.45 & 10.26\\
\hline
\multirow{2}{*}{Yoruba} & Central-English  &  21.46    &    18.10  \\
& Standard-English &  33.51  & 32.66 \\
\hline
\multirow{3}{*}{Tigrinya} & Eritrean   &  17.87    &      \\
& Ethiopian & 21.44 \\
\hline
\multirow{21}{*}{Basque} & Basque-English & 28.40 & 30.94 \\

& Mugerre-English   &    22.00   & 19.71  \\

& Maule-English  & 11.55 & 10.36\\
& Larzabale-English & 20.37 & 17.88\\
& Urruna-English  & 18.50 & 16.25 \\
& Heleta-English  &  22.53 & 22.03\\
& Uharte-English & 21.10 & 18.57 \\
& Bidarrai-English  & 17.93 & 17.00 \\
& Behorlegi-English & 24.19 & 21.35\\
& Iholdi-English & 16.68 & 15.01\\
& Baigorri-English & 20.21 & 18.80\\
& Suhuskune-English & 21.10 & 18.57\\
& Jutsi-English  & 21.46  & 20.00\\
& Garruze-English & 25.40 & 22.00 \\
& Senpere-English & 23.47 & 20.35 \\
& Sara-English & 23.04 & 20.25 \\
& Barkoxe-English & 10.92 & 10.82\\
& Luhuso-English  & 22.58 & 20.95\\
& Amenduze-English &  24.21 & 20.86\\
& Donibane-English & 20.28 & 18.03\\
& Azkaine-English & 25.61 & 22.58\\
& Jatsu-English & 17.00 & 14.56\\

\hline
\multirow{6}{*}{Bengali} & Barisal-English  & 11.33  & 12.68\\
& Dhakaiya-English  & 17.18 & 17.85\\
& Jessore-English  & 20.71 & 21.44\\
& Khulna-English & 18.96 & 19.73\\
& Kushtia-English  & 17.36 & 19.12\\
& Standard-English & \\

\end{longtable}
\twocolumn
\normalsize



\begin{longtable}{llrr}
\caption{MT Dialects without reference}
\label{tab:MT_without_reference}\\
\toprule
     Language group &      Dialect  &  NLLB-600M\_bleu & NLLB-1.3B\_bleu  \\
\midrule
\endfirsthead
%\caption[]{MT} \\

\multirow{21}{*}{Basque} & Mugerre  &     20.12 &     \\

& Maule  & 12.13 \\
& Larzabale & 19.64 \\
& Urruna  & 16.98\\
& Heleta  & 19.66\\
& Uharte & 17.96 \\
& Bidarrai  & 17.72 \\
& Behorlegi & 21.95 \\
& Iholdi & 15.95 \\
& Baigorri & 17.41 \\
& Suhuskune & 17.96 \\
& Jutsi  & 19.36 \\
& Garruze & 21.74 \\
& Senpere & 20.18 \\
& Sara & 20.34 \\
& Barkoxe & 13.46 \\
& Luhuso  & 20.74 \\
& Amenduze &  21.13 \\
& Donibane & 19.55 \\
& Azkaine & 21.81 \\
& Jatsu & 15.98 \\
\hline
\multirow{1}{*}{French} & Occitan  &    20.72   &  25.74    \\
\hline
\multirow{1}{*}{Farsi} & Dari  &   37.02   &   40.49   \\
\hline
\multirow{2}{*}{German} & Saxony  &  12.00    &  8.62    \\
& Danube\_Bavarian & 9.49  & 12.00\\
\hline
\multirow{2}{*}{Kurdish} & Mehabad  &  35.75    &  34.88    \\
& Sine &  22.56  & 22.59\\
\hline
\multirow{1}{*}{Greek} & Cretan  & 25.03     &   21.34   \\
\hline
\multirow{1}{*}{Griko} & Griko  &  3.92    & 3.97     \\
\hline
\multirow{3}{*}{Norwegian} & Setesdal & 2.24 & 4.22\\
& Southwestern &  21.88 & 15.81\\
& Eastern & 24.00 & 27.49\\
\hline





\end{longtable}
\twocolumn
\normalsize

==> dialectbench_language.tex <==
In \cref{fig:dial_count}, we list the language \clusters{} in \benchmark{} and the number of \dialects{} in each. Below, provide some more details about the languages, grouping them by family. In \cref{lang_list} of the Appendix, we describe all the \dialects{} in detail. 

\subsection{Indo-European} 

The Indo-European languages are spoken across the world and have the largest number of living speakers.\footnote{\url{https://en.wikipedia.org/wiki/List_of_language_families}} Accordingly, this family has the widest coverage of all families in our benchmark. In total, we cover 23 language \clusters{}: 6 Italic-Romance, 5 Germanic, 5 Indo-Iranian, 4 Balto-Slavic, as well as Albanian, Armenian, and Greek. \Dialects{} under this language family are covered by all 10 \benchmark{} tasks. 

%\oreva{to-do: say whether the dialects here are regional or not, or whether they are mutually intelligible} \ff{let,s put the list of language family subgroups in a table and describe here, their stand out features only (eg. indo-european has the widest coverage in our benchmark. In total195 we cover 26 language varieties)} \oreva{That sounds good} 
%\oreva{should we actually just put this section in a table?. "Family specific coverage" }

We discuss some language \clusters{} in this family in more detail below.

%as we only cover Central Kurdish varieties spoken in X and available in 4 tasks. 

%\DC{Some of these paragraphs are actually not saying that much and could be deleted}

\subsubsection{Italian} While they are largely recognized as distinct languages, we group together a number of closely related languages from the Italian peninsula. These languages (e.g., Neapolitan, Sicilian, Lombard, Sardinian) have substantial lexical similarity and mutual intelligibility with Italian, and in practice, they co-exist with standard Italian. We direct the reader to~\citet{ramponi-2023-italy} for a comprehensive overview of language technologies for the language varieties of Italy.

% \subsection{French} We group Franco-Provençal languages (e.g., Norman, Occitan, Walloon) with French as they are closely related to French and spoken in France. We also include the Franco-Provençal language Arpitan in this \cluster, though it is spoken in Italy.

\subsubsection{Portuguese}
For Portuguese, \benchmark{} includes both European and Brazilian dialects. Unfortunately, to our knowledge there are no publicly available annotated data for Portuguese from Mozambique, Angola, or other Portuguese-speaking regions. 

\subsubsection{Spanish}
Although Spanish is spoken in many different parts of the world, we found very little data clearly originating from Latin America, so we opted for a comparison with closely-related Ibero-Romance languages from the Iberian peninsula, like Galician and Mirandese.

\subsubsection{English} 
English is the world's most widely spoken language. We cover 11 country-level English dialects using the SD-QA transcribed question-answering dataset~\cite{faisal-etal-2021-sd-qa}. For token-level tasks such as Dependency Parsing and POS tagging, 
%\DC{define}\an{be specific}
we also include Singlish, which is a colloquial variety of English spoken in Singapore, with influence from Malay, southern Chinese dialects, and Tamil~\cite{wang-etal-2017-universal-fixed}. In addition, we include African-American Vernacular English (AAVE), spoken mostly by African-American communities in the United States (US). AAVE shares a large portion of its grammar and phonology with Southern US English from regions where the historical enslavement of African Americans primarily occurred~\cite{Thomas+2004+300+324}. We find a token-level dataset for AAVE originally derived from informal social media texts~\cite{blodgett-etal-2018-twitter}.

\subsubsection{Norwegian} 

Unlike other languages, this Indo-European language has two standard written varieties, with different ISO-639-3 codes: Bokmål (nno) amd Nynorsk (nob). This broad availability of written resources aided us to find evaluation and training data for a diverse range of tasks. There is another less-common written variety, Samnorsk, which was an attempt to fuse both of the two written varieties into one. We include NER task data for all these three written forms~\cite{johansen2019ner}. 

\subsection{Afro-Asiatic} 

This family is represented in \benchmark{} by varieties of Arabic and Tigrinya. 
Tigrinya is the smaller of the two, as we only cover the Eritrean and Ethiopian dialects in the MT task.

Arabic is a collection of roughly 30 vernaculars %~\cite{sil6393} and 28 countries use Arabic as their official language~\cite{tarjamaArabicDialects}. 
sharing a common written form, known as Modern Standard Arabic. Some prominent dialects include Egyptian, Maghrebi, Gulf, and Levantine Arabic.
All of the 10 tasks of \benchmark{} contain Arabic dialects, largely due to MADAR~\cite{bouamor-etal-2018-madar}, a large city-level Arabic corpus for machine translation and dialect identification. For the other tasks, we utilize the ample availability of independent country-level Arabic dialectal datasets. 

\subsection{Sino-Tibetan} 

This family is represented in \benchmark{} only by Chinese languages.
Standard written Chinese is based on Mandarin, and is categorized in the \benchmark{} datasets in a few different ways: as a single language, by region (mainland China vs.~Taiwan), or by writing system (simplified, which is used in mainland China, Malaysia, and Singapore, vs.~traditional, which is used in Taiwan, Hong Kong, and Macau).
Other Chinese dialects are also represented: Hakka and Minnan (including Taiwanese) using the Latin alphabet, and Wu (including Shanghainese), Yue (including Cantonese), and Classical Chinese using Chinese characters.
Note that these are mutually unintelligible with one another and with Mandarin \citep{tang-van-heuven-2009}.

\subsection{Other families and languages}

\insentpara{Uralic languages} \benchmark{} includes Finnish, Komi, Mari, and Sami language \clusters{}. 
%in \benchmark{} are Finnish, Sami, Estonian, Mari and Komi. %Sami varieties are the most closely related to the Finnic languages, Finnish and Estonian.\footnote{\url{https://en.wikipedia.org/wiki/S\%C3\%A1mi_languages}} 
Uralic languages are generally not mutually intelligible. 
%\an{This sentence makes it sound like we form a cluster with all Uralic languages -- but in practice we have clusters for each of these, no? Maybe rephrase the first sentence to "DialectBench includes Finish, Sami, ... clusters."}. \oreva{sounds good} 
Overall, we have 11 Uralic varieties covered by the 3 sequence labeling tasks (DEP, POS, and NER) in \benchmark. The POS task further includes 6 fine-grained varieties of the Finnish language \cluster. 

\insentpara{Turkic languages} are closely related to one another and have some mutual intelligibility through similar vocabulary, a shared word order and some phonological similarities \cite{mirzakhalov-etal-2021-large}. %\an{Good cite or relevant one might be the Turkish interlingua MT paper}. 
In \benchmark{} we cover 3 \dialects{} of Azerbaijani and 8 Turkic languages with the data presence in Machine Translation and NER. %\DC{does MT have the majority of languages or majority of data?}
%\DC{Azerbaijani is a \dialect{} of Turkish in the MT table, but its own language \cluster{} in the main table. Uzbek is ``orphaned'' in the MT table -- is it supposed to be under Turkish? Are all those languages really so close to Turkish as to be in the same \cluster{}?} \oreva{For MT, we grouped all turkic languages in \cite{mirzakhalov2021large} under the same \cluster{}, so they are more of closely related-languages.  } \DC{The discrepancy needs to be either fixed or explained.}

\insentpara{Northwest Caucasian languages} are represented in \benchmark{} by Adyghe and Kabardian. Kabardian is a very close relative of Adyghe and sometimes treated as a dialect of Adyghe. Our task coverage of this language family is only in NER.

\insentpara{Niger-Congo languages} in \benchmark{} are Sotho, Swahili and Yoruba. Swahili and Sotho are both Bantu languages, while Yoruba is in the Volta–Niger branch.

% \insentpara{Eskimo–Aleut languages} in \benchmark{} are Inuktitut and Kalaallisut in NER. 
%\oreva{more probably still needed to be said there}

\insentpara{Basque} is a language isolate spoken in southwestern Europe. Most of its \dialects{} are mutually intelligible \cite{trudgill1992ausbau}. In all, 22 \dialects{} are present in \benchmark{} in the MT task.

\insentpara{Guarani} is spoken in Paraguay and neighboring countries. It is the sole representative of the Tupian language family in \benchmark.

==> langlist_table.tex <==
\begin{table}
\tiny
\centering
\caption{\Dialects{} represented in DialectBench. 
\Dialects{} with (*) are generally considered to be closely-related languages rather than dialects. \Dialects{} superscripted by a task name have several fine-grained varieties represented by the task as shown in the relevant results table for that task.}
\label{lang_list}
\begin{tabular}{p{1cm}p{.2cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}}
\toprule
{} &  DEP  &  POS  &  NER &  EQA &  MRC &  NLI &  TC &  SA &  DId &  Total \\
\midrule
Total                        &           40 &           51 &   85 &   24 &   11 &   38 &  38 &   9 &   49 &    208 \\
arabic                       &            3 &            6 &    2 &    7 &    6 &    9 &   9 &   9 &   26 &     42 \\
anglic                       &            3 &            2 &    4 &   11 &    1 &    1 &   1 &   0 &    3 &     19 \\
sinitic                      &            3 &            3 &    6 &    0 &    2 &    3 &   3 &   0 &    4 &     13 \\
high german                  &            2 &            2 &    8 &    0 &    0 &    2 &   2 &   0 &    4 &     13 \\
southwestern shifted romance &            4 &            5 &    5 &    0 &    0 &    4 &   4 &   0 &    6 &     11 \\
greek                        &            0 &            0 &    2 &    0 &    0 &    0 &   0 &   0 &    6 &     10 \\
gallo-rhaetian               &            3 &            3 &    6 &    0 &    0 &    1 &   1 &   0 &    0 &      8 \\
neva                         &            0 &            8 &    0 &    0 &    0 &    0 &   0 &   0 &    0 &      8 \\
italian romance              &            4 &            4 &    4 &    0 &    0 &    2 &   2 &   0 &    0 &      7 \\
norwegian                    &            3 &            3 &    3 &    0 &    0 &    2 &   2 &   0 &    0 &      5 \\
gallo-italian                &            1 &            1 &    5 &    0 &    0 &    3 &   3 &   0 &    0 &      5 \\
common turkic                &            0 &            0 &    4 &    0 &    0 &    3 &   3 &   0 &    0 &      5 \\
komi                         &            3 &            3 &    2 &    0 &    0 &    0 &   0 &   0 &    0 &      4 \\
serbian-croatian-bosnian     &            0 &            0 &    4 &    0 &    0 &    0 &   0 &   0 &    0 &      4 \\
tupi-guarani subgroup i.a    &            3 &            3 &    0 &    0 &    0 &    0 &   0 &   0 &    0 &      3 \\
modern dutch                 &            0 &            0 &    3 &    0 &    0 &    1 &   1 &   0 &    0 &      3 \\
eastern romance              &            0 &            0 &    3 &    0 &    0 &    0 &   0 &   0 &    0 &      3 \\
frisian                      &            0 &            0 &    3 &    0 &    0 &    0 &   0 &   0 &    0 &      3 \\
kurdish                      &            0 &            0 &    2 &    0 &    0 &    2 &   2 &   0 &    0 &      3 \\
swahili                      &            0 &            0 &    0 &    2 &    0 &    0 &   0 &   0 &    0 &      3 \\
bengali                      &            0 &            0 &    0 &    2 &    0 &    0 &   0 &   0 &    0 &      3 \\
Other                        &            8 &            8 &   19 &    2 &    2 &    5 &   5 &   0 &    0 &     33 \\
\bottomrule
\end{tabular}
\end{table}

==> taxonomy.tex <==

\begin{figure*}
\small
    \centering
    
%
\tikzset{
    basic/.style  = {draw, text width=2cm, align=center, font=\sffamily, rectangle},
    root/.style   = {basic, rounded corners=2pt, thin, align=center, fill=green!30},
    onode/.style = {basic, thin, rounded corners=2pt, align=center, fill=green!60,text width=2.5cm,},
    tnode/.style = {basic, thin, align=left, fill=pink!60, text width=2.5cm, align=center},
    xnode/.style = {basic, thin, rounded corners=2pt, align=center, fill=blue!20,text width=2.5cm,},
    wnode/.style = {basic, thin, align=left, fill=pink!10!blue!80!red!10, text width=6.5em},
    cnode/.style = {basic, thin, align=center, rounded corners=1pt, fill=yellow!110!blue!50, rounded corners=2pt,draw=none, text width=2.5cm},
    edge from parent/.style={draw=black, edge from parent fork right}

}


% [Taxonomy, basic,  l sep=10mm,
%     [Data and Language, xnode,  l sep=10mm,
%         [Pretraining Data, tnode,  l sep=10mm,
%             [Parallel, onode, l sep=10mm,
%                 [\cite{conneau-etal-2020-unsupervised}, cnode]
%             ]
%             [Monolingual, onode , l sep=10mm,
%                 [~\cite{devlin-etal-2019-bert, brown2020language}, cnode]
%             ]
%         ]
%         [Language, tnode]
%     ]
% ]
%
\hspace{-2em}
\begin{forest} for tree={
    grow=east,
    growth parent anchor=west,
    parent anchor=east,
    child anchor=west,
    edge path={\noexpand\path[\forestoption{edge},->, >={latex}] 
         (!u.parent anchor) -- +(10pt,0pt) |-  (.child anchor) 
         \forestoption{edge label};}
}
% lsep is used for arrow distance
[Taxonomy, basic,  l sep=10mm,
    [Data , xnode,  l sep=10mm,
        [Type, tnode,  l sep=10mm,
            [dialectal, onode, l sep=10mm,
                % [\cite{conneau-etal-2020-unsupervised}, cnode]
            ]
            [regional/related, onode, l sep=10mm,]
            [historical, onode, l sep=10mm,]
            [non-native, onode, l sep=10mm,]
            [not applicable, onode, l sep=10mm,]
        ]
        [Form, tnode,  l sep=10mm,
            [raw, onode, l sep=10mm,
                % [\cite{conneau-etal-2020-unsupervised}, cnode]
            ]
            [audio, onode, l sep=10mm,]
            [text, onode, l sep=10mm,]
            [audio+text, onode, l sep=10mm,]
            [annotated, onode, l sep=10mm,]
            [contrastive, onode, l sep=10mm,]
            [lexicon, onode, l sep=10mm,]
            [synthetic, onode, l sep=10mm,]
            [dictionary, onode, l sep=10mm,]
            [system, onode, l sep=10mm,]
        ]
    ]
]
\end{forest}

    \caption{Area Taxonomy of Multilingual Text Representation}
    \label{fig:lit_surv}
\end{figure*}
